Multi-level Second-order Few-shot Learning

We propose a Multi-level Second-order (MlSo) few-shot learning network for supervised or unsupervised few-shot image classification and few-shot action recognition. We leverage so-called power-normalized second-order base learner streams combined with features that express multiple levels of visual abstraction, and we use self-supervised discriminating mechanisms. As Second-order Pooling (SoP) is popular in image recognition, we employ its basic element-wise variant in our pipeline. The goal of multi-level feature design is to extract feature representations at different layer-wise levels of CNN, realizing several levels of visual abstraction to achieve robust few-shot learning. As SoP can handle convolutional feature maps of varying spatial sizes, we also introduce image inputs at multiple spatial scales into MlSo. To exploit the discriminative information from multi-level and multi-scale features, we develop a Feature Matching (FM) module that reweights their respective branches. We also introduce a self-supervised step, which is a discriminator of the spatial level and the scale of abstraction. Our pipeline is trained in an end-to-end manner. With a simple architecture, we demonstrate respectable results on standard datasets such as Omniglot, mini-ImageNet, tiered-ImageNet, Open MIC, fine-grained datasets such as CUB Birds, Stanford Dogs and Cars, and action recognition datasets such as HMDB51, UCF101, and mini-MIT.

==> abstract.tex <==
\begin{abstract}
In this paper, we propose a novel few-shot similarity learning network for image classification and action recognition leveraging power normalizing second-order similarity network streams combined with multi-depth feature retracing and clustering mechanisms. As second-order pooling has advanced image recognition, we investigate several formulations capturing second-order statistics and existing Power Normalizations (PN), and we derive a sigmoid-like interpretable PN function. The goal of multi-depth retracing is to extract feature representations at different CNN depths to realize various levels of visual abstraction and thus allow a more robust similarity learning. Moreover, we propose to use a discriminator to classify the depth index of features and enhance the discrimination of multi-depth features. Our models are trained end-to-end to learn the similarity between the support and query images (or videos) for the problem of one- and few-shot learning. We demonstrate state-of-the-art results on standard datasets such as Omniglot, \textit{mini}-ImageNet, \textit{tiered}-ImageNet,, Open MIC, fine-grained datasets such as Flower102, CUB-200, Food-101, and action recognition datasets such as HMDB51, UCF101, and miniMIT.
\keywords{{Few-shot Learning \and Second-order Pooling \and Self-supervised Learning \and Image Classification \and Action Recognition}}
\end{abstract}

==> table.tex <==
{%\small
\begin{table*}[b]
%\centering
\caption{Evaluations on the Open MIC dataset (Protocol I). See our ArXiV for a challenging Prot. III ({\fontsize{9}{9}\selectfont \url{http://claret.wikidot.com}}).$\!\!\!\!\!$}
\label{table_o1}
\makebox[\textwidth]{
\setlength{\tabcolsep}{0.20em}
\renewcommand{\arraystretch}{0.90}
\fontsize{8.5}{9}\selectfont
\begin{tabular}{l|c|c|c|c|c|c|c|c|c|c|c|c|c}
\toprule
Model & $L$ & $p1\!\!\rightarrow\!p2$ & $p1\!\!\rightarrow\!p3$& $p1\!\!\rightarrow\!p4$& $p2\!\!\rightarrow\!p1$& $p2\!\!\rightarrow\!p3$ &$p2\!\!\rightarrow\!p4$& $p3\!\!\rightarrow\!p1$& $p3\!\!\rightarrow\!p2$& $p3\!\!\rightarrow\!p4$& $p4\!\!\rightarrow\!p1$& $p4\!\!\rightarrow\!p2$& $p4\!\!\rightarrow\!p3$\\
\hline
Relation Net \cite{sung2017learning} & \multirow{6}{*}{5} & $71.1  $ & $53.6  $ & $63.5  $ & $47.2  $ & $50.6  $ & $68.5  $ & $48.5  $ & $49.7  $ & $68.4  $ & $45.5  $ & $70.3  $ & $50.8  $\\
SoSN &  & $80.8   $ & $64.3   $ & $74.9   $ & $58.8   $ & $61.2   $ & $76.9   $ & $61.3   $ & $80.8   $ & $77.2   $ & $58.2   $ & $80.1   $ & $61.6   $\\
SoSN+SigmE &  & ${81.4}   $ & ${65.2}   $ & ${75.1}   $ & ${60.3}   $ & ${62.1}   $ & ${77.7}   $ & ${61.5}   $ & ${82.0}   $ & ${78.0}   $ & ${59.0}   $ & ${80.8}   $ & ${62.5}   $\\
{\fontsize{6}{7}\selectfont MdSoSN} &  & ${80.3}   $ & ${65.8}   $ & ${76.7}   $ & ${61.3}   $ & ${61.6}   $ & ${77.4}   $ & ${62.3}   $ & ${80.3}   $ & ${76.9}   $ & ${58.8}   $ & ${81.0}   $ & ${62.1}   $\\
{\fontsize{6}{7}\selectfont SoSN+SigmE(224x224)} &  & ${83.9}   $ & ${68.9}   $ & ${82.1}   $ & ${64.7}   $ & ${66.6}   $ & ${82.2}   $ & ${65.5}   $ & ${84.5} \!\pm\! 0.8$ & ${80.6} \!\pm\! 0.8$ & ${64.6}   $ & ${83.6} \!\pm\! 0.8$ & ${66.0}   $\\
{\fontsize{6}{7}\selectfont MdSoSN(224x224)} &  & ${85.9}   $ & ${72.4} \!\pm\! 1.2$ & ${83.2} \!\pm\! 1.0$ & ${66.7} \!\pm\! 1.2$ & ${70.0} \!\pm\! 1.2$ & ${84.2} \!\pm\! 1.0$ & ${70.6} \!\pm\! 1.2$ & ${85.7} \!\pm\! 0.8$ & ${82.4}   $ & ${67.1} \!\pm\! 1.3$ & ${84.3} \!\pm\! 0.8$ & ${67.4} $\\
{\fontsize{6}{7}\selectfont MdSoSN+GM(224x224)} &  & $\mathbf{86.1}   $ & $\mathbf{72.7} \!\pm\! 1.2$ & $\mathbf{83.6} \!\pm\! 1.0$ & $\mathbf{67.1} \!\pm\! 1.2$ & $\mathbf{70.5} \!\pm\! 1.2$ & $\mathbf{84.6} \!\pm\! 1.0$ & $\mathbf{71.1} \!\pm\! 1.3$ & $\mathbf{86.1} \!\pm\! 0.8$ & $\mathbf{83.0}   $ & $\mathbf{67.5} \!\pm\! 1.3$ & $\mathbf{84.8} \!\pm\! 0.8$ & $\mathbf{67.6} \!\pm\! 1.1$\\
\hline
Relation Net & \multirow{4}{*}{20} & $40.1   $ & $30.4   $ & $41.4   $ & $23.5   $ & $26.4   $ & $38.6   $ & $26.2   $ & $25.8   $ & $46.3   $ & $23.1   $ & $43.3   $ & $27.7   $\\
SoSN &  & $61.0   $ & $42.3   $ & $60.2   $ & $35.7   $ & $37.0   $ & $54.8   $ & $36.0   $ & $59.1   $ & $57.0   $ & $36.4   $ & $59.3 $ & $37.8   $\\
SoSN+SigmE &  &   ${61.5}   $ & ${42.5}   $ & ${61.0}   $ & ${36.1}   $ & ${38.3}   $ & ${56.3}   $ & ${38.7}   $ & ${59.9}   $ & ${59.4}   $ & ${37.4}   $ & ${59.0}   $ & ${38.6}   $\\
{\fontsize{6}{7}\selectfont SoSN+SigmE(224x224)} &  & ${63.6}   $ & ${48.7}   $ & ${65.6}   $ & ${42.6}   $ & ${43.9}   $ & ${61.8}   $ & ${43.7}   $ & ${63.3}   $ & ${63.5}   $ & ${43.2}   $ & ${62.5}   $ & ${43.7}   $\\
{\fontsize{6}{7}\selectfont MdSoSN(224x224)} &  & ${65.1}   $ & ${50.2}   $ & ${67.2}   $ & ${44.3}   $ & ${45.3}   $ & ${64.1}   $ & ${45.3}   $ & ${64.9}   $ & ${65.2}   $ & ${45.7}   $ & ${64.2}   $ & ${44.3}   $\\
{\fontsize{6}{7}\selectfont MdSoSN+GM(224x224)} &  & $\mathbf{65.4}   $ & $\mathbf{50.3}   $ & $\mathbf{67.5}   $ & $\mathbf{44.7}   $ & $\mathbf{45.5}   $ & $\mathbf{64.5}   $ & $\mathbf{45.6}   $ & $\mathbf{65.3}   $ & $\mathbf{65.3}   $ & $\mathbf{45.8}   $ & $\mathbf{64.5}   $ & $\mathbf{44.7}   $\\
\hline
%\arrayrulecolor{black} \cdashline{1-7}[1pt/3pt]
SoSN+SigmE & \multirow{2}{*}{30} &   $60.6   $ &  $40.1  $ & $58.3  $ & $34.5  $ & $35.1  $ & $54.2  $ & $36.8  $ & $58.6  $ & $56.6  $ & $35.9  $ & $57.1  $ & $37.1  $\\
{\fontsize{6}{7}\selectfont SoSN+SigmE+224x224} &   &   $61.7  $ &  $46.6  $ & $64.1  $ & $41.4  $ & $40.9  $ & $60.3  $ & $41.6  $ & $ 61.0  $ & $ 60.0  $ & $ 42.4  $ & $ 61.2  $ & $ 41.4  $\\
{\fontsize{6}{7}\selectfont MdSoSN(224x224)} &   &  ${62.3}  $ &  ${47.3}  $ & ${64.5}  $ & ${43.1}  $ & ${41.8}  $ & ${61.1}  $ & ${43.1}  $ & ${62.1}  $ & ${61.6}  $ & ${43.4}  $ & $ {61.9}  $ & ${42.7}  $\\
{\fontsize{6}{7}\selectfont MdSoSN+GM(224x224)} &   &  $\mathbf{62.5}  $ &  $\mathbf{47.6}  $ & $\mathbf{64.8}  $ & $\mathbf{43.5}  $ & $\mathbf{42.2}  $ & $\mathbf{61.2}  $ & $\mathbf{43.6}  $ & $ \mathbf{62.4}  $ & $\mathbf{62.9}  $ & $\mathbf{43.8}  $ & $ \mathbf{62.0}  $ & $\mathbf{43.1}  $\\
\hline
SoSN+SigmE & \multirow{2}{*}{45} &   $53.3  $ &  $37.3  $ & $54.6  $ & $30.8\!\pm\! 0.4$ & $ 32.4  $ & $ 52.4  $ & $ 32.1  $ & $ 54.2  $ & $ 51.1  $ & $ 30.5\!\pm\! 0.4$ & $ 51.9  $ & $33.4   $\\
\bottomrule
\end{tabular}}
p1: shn+hon+clv, p2: clk+gls+scl, p3: sci+nat, p4: shx+rlc. Notation {\em x$\!\rightarrow$y} means training on exhibition {\em x} and testing on {\em y}.
\end{table*}
}
